$P_c\varepsilon\kappa_{max}$-Means++: Adapt-$P$ Driven by Energy and Distance Quality Probabilities Based on $\kappa$-Means++ for the Stable Election Protocol (SEP)

The adaptive probability $P_{\text{\tiny{adp}}}$ formalized in Adapt-$P$ is developed based on the remaining number of SNs $\zeta$ and optimal clustering $\kappa_{\text{\tiny{max}}}$, yet $P_{\text{\tiny{adp}}}$ does not implement the probabilistic ratios of energy and distance factors in the network. Furthermore, Adapt-$P$ does not localize cluster-heads in the first round properly because of its reliance on distance computations defined in LEACH, that might result in uneven distribution of cluster-heads in the WSN area and hence might at some rounds yield inefficient consumption of energy. This paper utilizes \nolinebreak{$k$\small{-}means\small{++}} and Adapt-$P$ to propose \nolinebreak{$P_{\text{c}} \kappa_{\text{\tiny{max}}}$\small{-}means\small{++}} clustering algorithm that better manages the distribution of cluster-heads and produces an enhanced performance. The algorithm employs an optimized cluster-head election probability $P_\text{c}$ developed based on energy-based $P_{\eta(j,i)}$ and distance-based $P\!\!\!_{\psi(j,i)}$ quality probabilities along with the adaptive probability $P_{\text{\tiny{adp}}}$, utilizing the energy $\varepsilon$ and distance optimality $d\!_{\text{\tiny{opt}}}$ factors. Furthermore, the algorithm utilizes the optimal clustering $\kappa_{\text{\tiny{max}}}$ derived in Adapt-$P$ to perform adaptive clustering through \nolinebreak{$\kappa_{\text{\tiny{max}}}$\small{-}means\small{++}}. The proposed \nolinebreak{$P_{\text{c}} \kappa_{\text{\tiny{max}}}${\small{-}}means{\small{++}}} is compared with the energy-based algorithm \nolinebreak{$P_\eta \varepsilon \kappa_{\text{\tiny{max}}}${\small{-}}means{\small{++}}} and distance-based \nolinebreak{$P_\psi d_{\text{\tiny{opt}}} \kappa_{\text{\tiny{max}}}${\small{-}}means{\small{++}}} algorithm, and has shown an optimized performance in term of residual energy and stability period of the network.

==> Makefile <==
##
## A helper Makefile to build easychair-based articles
## under *nix environments with GNU make.
##
## Modify according to your needs.
##
## Author: Serguei Mokhov
## $Id: Makefile,v 1.5 2008/06/16 18:21:00 mokhov Exp $
##

#
# Settings
#

#PDFLATEXFLAGS = --interaction=batchmode --file-line-error-style
PDFLATEXFLAGS = --interaction=batchmode

DELIVERABLE = easychair
SUBMISSIONDIR = easychair-submission


#
# Build
#

all: letter a4
#all: $(DELIVERABLE).pdf

a4: $(DELIVERABLE)-a4.pdf
letter: $(DELIVERABLE)-letter.pdf

$(DELIVERABLE).pdf: $(DELIVERABLE).tex $(DELIVERABLE).bib $(DELIVERABLE).cls Makefile
	@echo "Compiling *.tex files..."
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)
	@echo "Compiling bibliography..."
	bibtex $(DELIVERABLE)
	@echo "Updating cross-references..."
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)

$(DELIVERABLE)-letter.pdf: $(DELIVERABLE).pdf
	cp $(DELIVERABLE).tex $(DELIVERABLE)-letter.tex
	cp $(DELIVERABLE).pdf $(DELIVERABLE)-letter.pdf
	@echo "US Letter build is done."

$(DELIVERABLE)-a4.pdf: $(DELIVERABLE).pdf
	@echo "Prepping A4 .tex file..."
	cat $(DELIVERABLE).tex | sed 's/\\documentclass{/\\documentclass[a4paper]{/g' > $(DELIVERABLE)-a4.tex
	@echo "Compiling *.tex files..."
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)-a4
	@echo "Compiling bibliography..."
	bibtex $(DELIVERABLE)-a4
	@echo "Updating cross-references..."
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)-a4
	pdflatex $(PDFLATEXFLAGS) $(DELIVERABLE)-a4
	@echo "A4 build is done."

submission: all
	mkdir -p $(SUBMISSIONDIR)
	cp Makefile *.tex *.bib *.pdf *.png *.jpg $(SUBMISSIONDIR)
	make -C $(SUBMISSIONDIR) clean
	tar cvf $(SUBMISSIONDIR).tar $(SUBMISSIONDIR)
	gzip --best $(SUBMISSIONDIR).tar

zip: all
	zip -9 $(DELIVERABLE).zip \
		$(DELIVERABLE).cls \
		$(DELIVERABLE).tex $(DELIVERABLE).bib \
		$(DELIVERABLE)-*.pdf *EC.pdf *.jpg \
		Makefile $(DELIVERABLE).tcp

#
# Clean up
#

clean:
	rm -f *~ *.log *.dvi *.aux *.toc \
          *.lot *.lof *.idx *.bbl *.blg *.ilg *.ind

maintainer-clean: clean
	rm -f $(DELIVERABLE).pdf $(DELIVERABLE)-a4* $(DELIVERABLE)-letter*

# EOF

